TANDEM: Learning Joint Exploration and Decision Making with Tactile Sensors

Inspired by the human ability to perform complex manipulation in the complete absence of vision (like retrieving an object from a pocket), the robotic manipulation field is motivated to develop new methods for tactile-based object interaction. However, tactile sensing presents the challenge of being an active sensing modality: a touch sensor provides sparse, local data, and must be used in conjunction with effective exploration strategies in order to collect information. In this work, we focus on the process of guiding tactile exploration, and its interplay with task-related decision making. We propose TANDEM (TActile exploration aNd DEcision Making), an architecture to learn efficient exploration strategies in conjunction with decision making. Our approach is based on separate but co-trained modules for exploration and discrimination. We demonstrate this method on a tactile object recognition task, where a robot equipped with a touch sensor must explore and identify an object from a known set based on binary contact signals alone. TANDEM achieves higher accuracy with fewer actions than alternative methods and is also shown to be more robust to sensor noise.

==> sections/definition.tex <==
\section{Problem Definition}

We want to train an efficient tactile exploration policy and we demonstrate our framework on tactile object recognition task. The task is to identify the object from a set of known objects using only tactile sensory feedback. We want the robot to be able to accurately identify the object with as little movement as possible. Thus, the performance is measured by both accuracy and number of actions executed by the robot. 


Our tactile finger moves on a 2D plane and is always perpendicular to the plane (Fig.~\ref{fig:teaser}). We make the assumption that the target object is placed roughly at the center of the workspace with any random orientations. The object is fixed and it does not move after interaction with the finger. At each time step $t$, the robot can execute an action $a_t \in \mathcal{A} = \{\text{up, right, down, left}\}$ which corresponds to a 5mm translation in the 4 directions on the plane. After each action, the robot receives a binary tactile signal $s_t \in \{0, 1\}$, where 0 indicates collision and 1 indicates collision-free. The robot at each time step needs to (1) encode the sequence of binary collision signals, (2) predict the label of the object, and (3) decide whether to terminate the episode based on its confidence level.

% We are using the Disco finger~\cite{piacenza2020sensorized}, mounted on a UR5 arm, as shown in Fig~\ref{fig:teaser}. Disco finger is optics-based multicurved robotic finger from which collision information can be extracted. The finger moves on a 30cm by 30cm 2D plane and is always perpendicular to this plane. We make the assumption that the target object is placed roughly at the center of the workspace with any random orientations. At each time step $t$, the robot can execute an action $a_t \in \{\text{up, right, down, left}\}$ which corresponds to a 5mm translation in the 4 directions on the plane. After each action, the robot receives a binary tactile observation $o_t \in \{0, 1\}$, where 0 indicates collision and 1 indicates collision-free. The robot at each time step needs to (1) encode the sequence of binary collision signals, (2) predict the label of the object, and (3) decide whether to terminate the episode based on its confidence level.


==> sections/simtoreal.tex <==
\subsection{Sim-to-real Adaptation}

We co-train a discriminator and explorer in the simulator and then evaluate the performance in both simulation and on real robots. Since we do not fine-tune our model on real robots, there is a sim-to-real gap when transferring our model trained in simulator to the real robot. We summarize the four categories of sim-to-real gaps and our methods to address them.

\subsubsection{Control} This comes from moving the robot arm in the real world setup. In simulation, we have precise control of the floating finger but on the real robots, we execute the 5mm action with five 1mm steps, so that the robot can subscribe to the tactile feedback after each small step to achieve closed-loop control. The challenge comes from precisely moving the finger for 1mm distance and also from the inverse kinematics solver to maintain the finger perpendicular to the workspace plane. The accumulated error in control for each episode on the real robot is around 5mm.

\subsubsection{Sensor} This noise comes from the tactile finger where a collision happens but is not detected, and vice versa. Our tactile finger contains a neural network that is trained to detect collision from the raw optic signals. Based on our analysis, the chance of such sensor error happening is around 0.3\% - 0.5\%. In order to handle the sensor noise, we apply 0.5\% sensor failure in our co-training process. 

\subsubsection{Object Position} We assume that the target object is always located at the center of the workspace; however, it is impossible to perfectly align the center of these random polygon shapes at the center of the workspace. In order to overcome this, we apply a random translation between -1cm to 1cm to both the $x$ and $y$ coordinates of the objects during training. 
%Thus, the discriminator is robust to translation noise of the object on the real robot experiments.

\subsubsection{Geometry} Even though the object is located at the same location in simulation and in real world, the target object might have a different ground truth occupancy grid. This can be a result of two reasons. (1) The real robot finger height does not perfectly match that of the simulator so that the location on the hemisphere tip touching the object is different. This makes the geometry shape of the object in real world shrunk / grown compared to that in the simulator. (2) In order to do collision checking in simulator, we run convex decomposition on the random polygons so that they are a union of convex sub-parts. This approximation process can introduce extra geometry discrepancy. 


